STCF Conceptual Design Report: Volume 1 -- Physics & Detector

The Super $\tau$-Charm facility (STCF) is an electron-positron collider proposed by the Chinese particle physics community. It is designed to operate in a center-of-mass energy range from 2 to 7 GeV with a peak luminosity of $0.5\times 10^{35}{\rm cm}^{-2}{\rm s}^{-1}$ or higher. The STCF will produce a data sample about a factor of 100 larger than that by the present $\tau$-Charm factory -- the BEPCII, providing a unique platform for exploring the asymmetry of matter-antimatter (charge-parity violation), in-depth studies of the internal structure of hadrons and the nature of non-perturbative strong interactions, as well as searching for exotic hadrons and physics beyond the Standard Model. The STCF project in China is under development with an extensive R\&D program. This document presents the physics opportunities at the STCF, describes conceptual designs of the STCF detector system, and discusses future plans for detector R\&D and physics case studies.

==> 06_01_Rvalue.tex <==
\subsubsection{R-value}
The $R$ value is defined as
\begin{equation}
   R(s) = \frac{\sigma_{\rm tot} ( e^+ e^- \to \gamma^* \to  {\rm hadrons)}}{\sigma (e^+e^-\to \gamma^* \to \mu^+ \mu^-)},
\end{equation}
which is a function of $s$. This quantity plays an important role in determining the running of electroweak coupling and in the study of precision
tests of SM. This can be seen in a recent study of global SM-fit\cite{Gfit}. $R(s)$ is also important for $g$-2 problem.
It is absolutely clear that more precise results on the $R$-value will be obtained at STCF.


==> 06_02_Inclusive.tex <==
\subsubsection{Inclusive Production of Single Hadron}

For large enough $\sqrt{s}$ the inclusive production of single hadron in $e^+e^- \to h +X$ can be predicted from QCD
with QCD factorization theorem\cite{Book}:
\begin{eqnarray}
\frac{d\sigma (e^+ e^- \rightarrow h +X)} {d z}  &=& \sum_{a=q,\bar q ,g} \int \frac{d\xi}{\xi} H_a (\frac{z}{\xi},Q^2,\mu^2) D_{a\rightarrow h} (\xi,\mu^2)
\nonumber\\
 &=& \sum_q \sigma (e^+ e^- \rightarrow q\bar q) \biggr ( D_{q\rightarrow h} (z) +   D_{\bar q\rightarrow h} (z) \biggr ) + {\mathcal O}(\alpha_s),
\label{FF}
\end{eqnarray}
where $z$ is the fraction of the energy carried by the observed hadron $h$. $H_a (a=q,\bar q,g)$ are functions which can be calculated
with perturbation theory. $D_{a\rightarrow h}$'s are parton fragmentation functions describing hadronization of a parton $a$ to $h$.
Eg.(\ref{FF}) is the statement from QCD collinear factorization.
The fragmentation functions are universal for any process where the QCD factorization is applicable. Extracting fragmentation functions
at rather low energy like the energy region of STCF around 4-5~GeV is specially important for the information about hadronization, because from the extracted fragmentation
functions one can test their energy evolution from a rather low energy scale to high energy scales.


==> 06_04_FF.tex <==
\subsubsection{Form Factors near Threshold}

{\color{red}
After 100 years of experimental studies, the structure of nucleons is still poorly understood.\cite{Nayak,Yang}
Now, time-like measurements are playing an increasingly important role.
Time-like pair-production measurements are not restricted to nucleons;
form-factors of all of the weakly decaying hyperons can be measured and compared, thereby opening a new, previously
unexplored dimension. Currently available
(statistically limited) time-like experiments demonstrate puzzling features in their threshold cross sections
and electric and magnetic form factors\cite{LarsOlsen:2020dpi}. At STCF, time-like nucleon and hyperon
form-factors  will be measured for $Q^{2}$ values as high as 40~GeV$^{2}$ with precisions that match
existing space-like region results for the proton \& neutron. Because the energy region
of STCF
the extracted form factors may not be at the energy scale at which perturbative QCD of exclusive processes works. However,
the behavior near the threshold is important for extracting information about the interaction between a baryon and antibaryon.
In the decay $J/\psi \to \gamma  p \bar p$
the enhancement has been observed by BES\cite{BES1} near the threshold of the $p\bar p$ system. Babar has reported the enhancement in the process
$e^+ e^- \to p\bar p, \Lambda \bar \Lambda, \Sigma^0 \bar \Sigma^0$\cite{BaB}, respectively. Likely, such an enhancement
is a common phenomenon near threshold. At STCF one can study this enhancement more precisely, and can extend the study to the system of $\Lambda_c \bar \Lambda_c$ to see if the enhancement happens in heavy baryon and antiheavy baryon system.}


==> Chapters/Chapter_02_Experimentalconditions/02_01_en_MDI.tex <==
\section{MDI and Luminosity Monitoring}

\subsection{Interaction Region}
The interaction region is the connector of the detector and the accelerator. So the geometry of accelerator elements and detector should be carefully considered in this region. The first final focus magnet is a crucial element for accelerator design. 
%test
%\input{08_01_Darksector}
%\input{08_02_MilliCharge}
%\input{08_ref_NewPhys}

